An Error-State Model Predictive Control on Connected Matrix Lie Groups for Legged Robot Control

This paper reports on a new error-state Model Predictive Control (MPC) approach to connected matrix Lie groups for robot control. The linearized tracking error dynamics and the linearized equations of motion are derived in the Lie algebra. Moreover, given an initial condition, the linearized tracking error dynamics and equations of motion are globally valid and evolve independently of the system trajectory. By exploiting the symmetry of the problem, the proposed approach shows faster convergence of rotation and position simultaneously than the state-of-the-art geometric variational MPC based on variational-based linearization. Numerical simulation on tracking control of a fully-actuated 3D rigid body dynamics confirms the benefits of the proposed approach compared to the baselines. Furthermore, the proposed MPC is also verified in pose control and locomotion experiments on a quadrupedal robot MIT Mini Cheetah.

==> method.tex <==
Supposing the input influence matrix $\mathcal{G}_k$ in output trajectory tracking control law \eqref{FTScontroller}  is unknown, we can formulate a constrained optimization problem to design the control input $u_k$ and the input influence matrix $\mathcal{G}_k$ concurrently. The finite-time stable tracking control law can be formulated as an equality constraints of a min norm controller:

\begin{equation}
    \begin{array}{c}
    \underset{\mathcal{G}_k, u_k}{\min} \|u_k\|_2^2 + w \|\mathcal{G}_k\|^2_{F} \\
    \mathcal{G}_k u_k=f_k \\
    % u_k \in \mathcal{U}, \mathcal{G}_k \in \mathcal{G} \\
    u_{\min} \le u_k \le u_{\max}, \\
    \|\mathcal{G}_{k} - \mathcal{G}_{k-1}\|_F\le L\|y_{k} - y_{k-1}\| \\
    sign(\mathcal{G}_{k}^{i,j})=s_{i,j}
    \end{array}
\end{equation}
where $w$ is a small positive weight to prevent $G_k$ from going to $0$. $u_{\min}$ and $u_{\max}$ are the lower and upper bounds of the control input. We also constrain the $\mathcal{G}_k$ to be Lipschitz continuous. Note that constraints on the sign of $\mathcal{G}_k$ is necessary. If we replace $\mathcal{G}_k$ with $-\mathcal{G}_k$, $-u_k$ then becomes the solution, which may not regulate the tracking error but amplifying it. 

TODO: We have to estimate the bounds of the tracking error here.
